Qd-tree: Learning Data Layouts for Big Data Analytics

Corporations today collect data at an unprecedented and accelerating scale, making the need to run queries on large datasets increasingly important. Technologies such as columnar block-based data organization and compression have become standard practice in most commercial database systems. However, the problem of best assigning records to data blocks on storage is still open. For example, today's systems usually partition data by arrival time into row groups, or range/hash partition the data based on selected fields. For a given workload, however, such techniques are unable to optimize for the important metric of the number of blocks accessed by a query. This metric directly relates to the I/O cost, and therefore performance, of most analytical queries. Further, they are unable to exploit additional available storage to drive this metric down further. In this paper, we propose a new framework called a query-data routing tree, or qd-tree, to address this problem, and propose two algorithms for their construction based on greedy and deep reinforcement learning techniques. Experiments over benchmark and real workloads show that a qd-tree can provide physical speedups of more than an order of magnitude compared to current blocking schemes, and can reach within 2X of the lower bound for data skipping based on selectivity, while providing complete semantic descriptions of created blocks.

==> sections/greedy_bak.tex <==
 \section{Greedy Construction of \qdrt}\label{sec:greedy}
% \subsection{Algorithm}

\revision{The \qdrt construction problem is an NP-hard combinatorial optimization problem. Greedy algorithms are a typical method to solve such problems; they are usually efficient and make locally optimal choices that which may result in long-term quality. Therefore, we start by proposing} a top-down greedy algorithm to construct the \qdrt. 
 We begin with all the tuples in a single block, i.e., the \qdrt has a single root node that contains all the tuples. In each iteration, we split a leaf node whose size is larger than $2b$ into two child nodes, and make sure the two children have size at least $b$. When choosing the cut for a node, we use the one that maximizes $C(T)$, i.e., the number of tuples skipped by the partitioning $\mathcal{P}_T$ induced by \qdrt $T$. 
 The idea is similar to the construction of a decision tree, except that in decision tree learning, the predicate is chosen using a different criterion such as information gain. 
 
 To present the algorithm, we define an action $a=(p,n)$ as applying cut $p$ to node $n$ in a \qdrt $T$. The result of action $a$ is denoted as $T\oplus a=T\oplus (p,n)$. In $T\oplus a$, node $n$ becomes the parent of two child nodes: the left child $n^p$  contains all the tuples in $n$ satisfying $p$, and the right child $n^{\neg p}$ contains all the tuples in $n$ satisfying $\neg p$. 
%  \todo{Before we go into formalism and proofs, should we discuss pseudocode of the greedy algorithm?  The above sentence ``When choosing the cut...'' may be too succinct of an algorithmic description?}
 \begin{algorithm}
 \caption{Greedy construction of \qdrt}
 \label{algo:greedy}
 \begin{algorithmic}
 \State \textbf{Input}: Tuple set $V$, min block size $b$, workload $W$, candidate cut set $P$
%  \Output{\qdrt $T$}
 \State \textbf{Initializatioin}: Set $T_0\gets V, t\gets 1$, $CanSplit \gets True $
 \While{$CanSplit$}
    \State $CanSplit \gets False $
    \For{each node $n\in T_{t-1}$ on the last level}
        \If{$n.size\ge 2b$} 
            \State $p\gets\arg\max_{p\in P,|n^p|\ge b, |n^{\neg p}|\ge b}C(T_{t-1}\oplus(p,n))$
            \If{$C(T_{t-1}\oplus(p,n))>C(T_{t-1})$}
                \State $T_{t}\gets T_{t-1}\oplus(p,n)$
                \State $t\gets t+1, CanSplit \gets True $
            \EndIf
        \EndIf
    \EndFor
 \EndWhile
 Return $T_{t-1}$
 \end{algorithmic}
 \end{algorithm}
 
 Our algorithm is presented in Algorithm~\ref{algo:greedy}. The main computation is to choose the cut $p$ that maximizes the greedy criterion $C(T_{t-1}\oplus(p,n))$ for each node $n$. For each level of the tree, the cost to executed the for loop is bounded by $O(|V||P|)$. The total cost of the while loop is bounded by $O(|V||P|d)$, where $d$ is the final depth of the tree. $\log_2 \frac{|V|}{b}\le d<|V|/b$. In the worst case, when the tree is least balanced, the complexity is quadratic to $|V|$. In the balanced case, the complexity grows as $|V|\log |V| $. If the number of partitions $|V|/b$ is a constant, then the cost is linear to $|V|$. 
 
 \subsection*{Approximation Guarantee}
 Under certain generic assumptions, we can prove that the greedy algorithm has a multiplicative offline approximation guarantee, and an additive online approximation guarantee. To the best of our knowledge, this the first algorithm with such guarantees. Our proof technique defines a new notion of submodularity: tree submodularity. We are unaware of notions of similar kind in other tree construction algorithms.
 
 Let $t$ be the number of leaf nodes in a \qdrt. The total number of nodes is $2t-1$. While the result of the greedy algorithm is invariant to the order of leaf splitting (which leaf to choose to split at each iteration), we fix the order to be top-down, left-to-right for ease of analysis. In each iteration $i$, a cut $p_i$ is chosen for the leftmost node $n_i$ on level $l_i$. We define this action as $a_i=(p_i,n_i)$. 
To characterize the properties of $C(T)$, it is useful to define 
two encodings of the \qdrt.
{
 \begin{definition}[Level-wise Encoding]
 A level-wise encoding $E(T)=\{n_i\}_1^{2t-1}$ of a \qdrt indexes all the nodes in a top-down, left-to-right order: $\forall 1\le i<j\le 2t-1$, node $n_i$ is either on top of node $j$, or on the left of node $j$ at the same level.
 \end{definition}
 }
 \begin{definition}[Action Encoding]
 An action encoding $A(T)=\{a_i\}_1^{t-1}$ of a \qdrt is the sequence of cuts chosen following the top-down, left-to-right order. We denote the tree after iteration $r$ as $T_r$, and $T_r=T_0\oplus a_1\oplus \dots \oplus a_r=T_0\oplus A_r(T)$. 
 \end{definition}
  After applying action $a_i$, a leaf node is split into two child nodes, which are appended to the end of the level-wise encoding. By definition, $T=T_{t-1}=T_0\oplus A_{t-1}(T)$.
 {
  \begin{lemma}[Tail Monotonicity]\label{lemma:monotonic}
  Given two \qdrt $T$ and $T'$, if $E(T)$ is a prefix of $E(T')$, then $C(T)\le C(T')$.
 \end{lemma}
 Lemma~\ref{lemma:monotonic} ensures that during the construction of \qdrt, the objective keeps increasing. 
 }
 To further characterize the structure of $C(T)$, 
 we define the following notion of concatenation of two trees.
 \begin{definition}[Action-based tree concatenation]
 Given two \qdrt $T$ (with $t$ leaf nodes) and $T'$, the action-based tree concatenation $T\oplus T'$ is defined as replacing the leftmost leaf node $n_t$ on level $l_{t}$ in $T$ with a subtree $n_t\oplus A(T')$. That is, the concatenation is obtained by applying the sequence of cuts in $T'$ to the next leaf node to split in $T$.
 \end{definition}
 {
 \begin{lemma}[Head Monotonicity]\label{lemma:head}
 Given two \qdrt $T$ (with $t$ leaf nodes) and $T'$, $C(T')\le C\left(T\oplus_{i=1}^t T' \right)$.
 \end{lemma}
 This lemma is true because every leaf node in $T\oplus_{i=1}^t T'$ contains a subset of tuples of a leaf node in $T'$.
 }
 \begin{definition}[Tree Submodularity]\label{def:submodular}
 Given two nodes $n$ and $n'$ in \qdrt $T$, and actions $a=(p,n),a'=(p,n')$. If $n'$ is an ancestor of $n$, let $T'$ be $T$ minus all descendants of $n'$. We say a \qdrt space is tree-submodular if for any such $T,n,n',a$ in the space, $C(T\oplus a)-C(T)\le C(T'\oplus a')-C(T')$.
 \end{definition}
 This property means that applying a cut in \qdrt has a diminishing return as the tree grows deeper. Let $Q(p)\subseteq W$ be the set of queries that can be skipped by $p$. We have the following sufficient condition for the \qdrt space to be tree-submodular. 
 \begin{lemma}\label{lemma:submodular}
 The \qdrt space is tree-submodular if the conjunction of cuts $p_1$ and $p_2$ cannot skip any query besides $Q(p_1)\cup Q(p_2)$ for all candidate cuts $p_1$ and $p_2$.
%  for any cut $p$ and query $q\in W$ such that $p$ cannot skip $q$ (i.e., $q$ intersects with both $p$ and $\neg p$), there does not exist a set of cuts $P$ such that $\bigwedge_{p'\in P}p'$ cannot skip $q$ and $\bigwedge_{p'\in P}p'\bigwedge p$ can skip $q$.
 \end{lemma}
 For example, if the workload $W$ only consists of conjunctive range queries, and each cut is a range predicate, the above condition is satisfied. 
 {
 \begin{proof}
 Let $n'$ be an ancestor node of $n$. We define the set of queries that can be skipped by $n$ as $Q_n\subseteq W$. It is easy to see $Q_{n'}\subseteq Q_{n}$. Let $Q(n,p)$ and $Q(n,\neg p)$ be the sets of queries skipped by the left and right child of $n$, and $c(n,p)$ be the number of tuples in node $n$ satisfying $p$. We then have:
 \begin{align}
     &C(T\oplus a)-C(T) \nonumber\\
                       =&c(n,p)|Q(n,p)\setminus Q_n|  +c(n,\neg p)|Q(n,\neg p)\setminus Q_n|\nonumber\\
                       =&c(n,p)|Q(p)\setminus Q_n|    +c(n,\neg p)|Q(\neg p)\setminus Q_n|\label{eq:sub1}\\
                    \le &c(n',p)|Q(p)\setminus Q_{n'}|+c(n',\neg p)|Q(\neg p)\setminus Q_{n'}|\\
                       =&c(n',p)|Q(n',p)\setminus Q_n|+c(n',\neg p)|Q(n',\neg p)\setminus Q_n|\label{eq:sub2}\\
                       =&C(T'\oplus a')-C(T')\nonumber
 \end{align}
 Both Eq.~\eqref{eq:sub1} and~\eqref{eq:sub2} use the sufficient condition.
 \end{proof}
 }
 
 \begin{theorem}
 If the \qdrt space is tree-submodular, the greedy top-down construction algorithm produces a \qdrt $T$ whose overall skipping capacity $C(T)$ is no worse than: 
 
 (a) $OPT-\frac{2|V|}{b}\left(C(T)-C(T^{-1})\right)$
 
 (b) $\left(1-\frac{b}{|V|}^{\frac{b\log_2 e}{2|V|}}\right) OPT$
 
 where $OPT$ refers to the skipping capacity of the optimal \qdrt $T^*$, and $T^{-1}$ refers to the sub \qdrt in $T$ by removing all the leaf nodes.
 \end{theorem}
 Bound (a) is an online bound because it depends on the algorithm output $C(T)$ and $C(T^{-1})$. Bound (b) is an offline bound independent of the algorithm output.
 {
 \begin{proof}
 Define $T^0=T$ and $T^{-i}=(T^{-(i-1)})^{-1}$ recursively. Let $t_i$ be the number of leaf nodes in $T^{-i}$. Let $A(T^*)=\{a^*_j\}_{j=1}^{t^*-1}$ be the action encoding of $T^*$. 

 From Lemma~\ref{lemma:head} we know:
 \begin{align*}
 &C(T^*)\le C\left(T^{-1}\oplus_{i=1}^{t_1} T^* \right)=C\left(T^{-1}\oplus_{i=1}^{t_1-1} T^*\oplus T^* \right)\\
 =&C\left(T^{-1}\oplus_{i=1}^{t_1-1} T^*\oplus A_{t*-2}(T^*)\oplus a^*_{t^*-1} \right)\\
 =&C\left(T^{-1}\oplus_{i=1}^{t_1-1} T^*\oplus A_{t*-2}(T^*)\right)\\
 +&C\left(T^{-1}\oplus_{i=1}^{t_1-1} T^*\oplus A_{t*-2}(T^*)\oplus a^*_{t^*-1} \right)\\
 -&C\left(T^{-1}\oplus_{i=1}^{t_1-1} T^*\oplus A_{t*-2}(T^*)\right)\\
  \end{align*}
Applying tree submodularity, we have:
\begin{align*}
 &C(T^*)\\
 \le& C\left(T^{-1}\oplus_{i=1}^{t_1-1} T^*\oplus A_{t*-2}(T^*)\right)
 +C\left(T_{t_0-2}\oplus a^*_{t^*-1} \right)
 -C\left(T_{t_0-2}\right)\\
  \end{align*}
Given the greedy criterion of choosing cuts during the construction of $T$, we know:
\begin{align}
    C\left(T_{t_0-2}\oplus a^*_{t^*-1} \right) \le C\left(T_{t_0-1}\right)
\end{align}
Therefore,
\begin{align}
 &C(T^*)\le C\left(T^{-1}\oplus_{i=1}^{t_1-1} T^*\oplus A_{t*-2}(T^*)\right)
 +C\left(T_{t_0-1}\right)-C\left(T_{t_0-2}\right)
\end{align}
Applying the same derivation for $A_{t*-j}(T^*), j=2,\dots,t^*-1$, we have:
\begin{align}
 &C(T^*)\le C\left(T^{-1}\oplus_{i=1}^{t_1-1}T^*\right)
 +(t^*-1)(C(T_{t_0-1})-C(T_{t_0-2}))
\end{align}
Repeating the above derivation for $T^{-1}\oplus_{i=1}^{t_1-j}T^*,j=1,\dots,t_1-1$, we have:
\begin{align}
\label{eq:t-1}
 &C(T^*)\le C\left(T^{-1}\right)
 +(t^*-1)(C(T^{0})-C(T^{-1}))
\end{align}
Since the minimal block size is $b$, the number of leaf nodes in $T^*$ is bounded by $|V|/b$. So $t^*\le 2|V|/b-1$.
Eq.~\eqref{eq:t-1} implies:
\begin{align*}
    C(T)&\ge C(T^*)-(t^*-2)(C(T)-C(T^{-1}))\\
    &>OPT-\frac{2|V|}{b}\left(C(T)-C(T^{-1})\right)
\end{align*}
So bound (a) is proved.

Eq.~\eqref{eq:t-1} also implies:
\begin{align*}
    C(T^*)-C(T^{-1})\le (t^*-1)(C(T^{0})-C(T^{-1}))
\end{align*}
Define $\Delta_i = C(T^*)-C(T^{-i})$, we have:
\begin{align*}
    &\Delta_1\le (t^*-1)(\Delta_1-\Delta_0)\\
\Rightarrow & \Delta_0\le \left(1-\frac{1}{t^*-1}\right)\Delta_1
\end{align*}
And similarly,
\begin{align}
    \Delta_i\le \left(1-\frac{1}{t^*-1}\right)\Delta_{i+1}
\end{align}
Assuming the depth of $T$ is $d$. We have $C(T^{-d})=0$, and $d\ge \log_2 \frac{|V|}{b} $.
\begin{align*}
    C(T^*)-C(T) &= \Delta_0 \le (1-\frac{1}{t^*-1})^d\Delta_d\\
    & \le e^{-\frac{d}{t^*-1}} C(T^*)< \left(\frac{b}{|V|}\right)^{\frac{b\log_2 e}{2|V|}}C(T^*)
\end{align*}
So bound (b) is proved.
 \end{proof}
 
 From the proof and the complexity analysis earlier, we see that the depth $d$
 of the tree plays a role in both algorithm complexity and approximation
 guarantee. The cost of the algorithm grows linearly with $d$, while the
 approximation ratio improves exponentially with $d$. The depth increases as the
 minimal block size $b$ decreases. The smaller the block size, the slower is the
 construction and the better the approximation guarantee.}
% LocalWords:  CanSplit Eq eq


==> sections/opt.tex <==
\section{Framework Extensions}
\label{sec:opt}

Having described two algorithms to construct a \qdrt in previous sections, we are now in position to
discuss extensions to our framework.

\subsection{Advanced Cuts}
Thus far we have assumed the candidate cuts are single-column predicates (Section~\ref{sec:allowed-cuts}).
They are desirable because their simplicity allows for fast evaluation during tree construction.
Nevertheless, \qdrt can be extended to support binary cuts of the form
\textsf{(attr1, op, attr2)}, as follows.

Recall from Table~\ref{table:node-metadata} there are two components of a node's
semantic description, and neither of them can describe a binary cut.  We append
a new component to each node $n$'s description:
\[
\textsf{n.adv\_cuts:} \quad \text{a bit vector of size |AC|}
\]
where the constant $|AC|$  denotes the number of \emph{advanced cuts} to support
and is specified for each workload a priori.  Each position $i$ corresponds to
``does this node contain records that satisfy advanced cut $i$'', with zero
indicating no and one indicating potentially yes.  This is the same semantics as \textsf{categorical\_mask}.

For instance, the TPC-H workload contains non-join binary filters such as:
\begin{itemize}
  \item $AC_0$: \texttt{c\_nationkey = s\_nationkey}
  \item $AC_1$: \texttt{l\_shipdate < l\_commitdate}
  \item $AC_2$: \texttt{l\_commitdate < l\_receiptdate}
\end{itemize}
A vector of $(0, 1, 1)$ thus indicates the first condition is definitely not met
(i.e., it describes a subspace of records whose \texttt{c\_nationkey} does
\emph{not} equate \texttt{s\_nationkey}).

\begin{table}[htp]\centering \small%
\begin{tabular}{@{} l l l @{}} \toprule
  &  w/o advanced cuts &  all cuts  \\ \midrule
Greedy \qdrt & 4.07\% & 2.57\%    \\
RL \qdrt &  3.97\% & 2.35\% \\ \bottomrule
\end{tabular}
\caption{\small Ablation study: how search space affects the quality of layout in terms of percentages of tuples accessed (lower is better). Detailed TPC-H workload setup is discussed in Section~\ref{sec:eval-setup}.\label{table:allowed-cuts}}
\end{table}

Table~\ref{table:allowed-cuts} shows an ablation study on the impact of
including these three special cuts into the search space.  We observe an up to
$1.68\times$ better quality for the layouts produced by Greedy and RL.  This makes sense,
as the three advanced cuts enlarge the search space and they are low-selectivity cuts
to start with (especially $AC_0$).

Lastly, the same mechanism also handles LIKE predicates or even stateless UDFs
(with the caveat that, clearly, the cost of evaluating the predicates depends on their inherent complexities).
The user can impose a limit on the maximum number of advanced cuts to support.

\subsection{Data Overlap}

With the abundance of cheap storage in the cloud, one desirable feature for an
analytics system is to trade space for potentially faster execution time.  A
fruitful line of work has dedicated to this problem, e.g., materialized views,
which we review in related work.  We now discuss how \qdrt can also naturally
support duplicating data.

Figure~\ref{fig:propeller} shows a 2D synthetic dataset and four queries.
Naively invoking either Greedy or \sys to construct a \qdrt for this
dataset-workload is suboptimal.
Any sequence of cuts---recall, the cut points are query literals, i.e., any of the edges in
the figure---would lead to 4 blocks: one with N+1 record, and three with N
records.  (This is due to the binary nature of the cuts.)  The three blocks would have to fetch the singleton record they need
from the first block.  Hence, a total of $3N$ extra tuples are read.

We extend \qdrt construction to handle such data overlap cases as follows.
Observe that the reason the ``lucky'' $(N+1)$-record block is not further cut is
due to the minimum block size constraint, $b$, usually set to tens of thousands.
We can instead launch either of our construction algorithms with a relaxed cutting condition: allowing one of the children to have size smaller than $b$.  With this change the lucky block would be further cut
into an $N$-record one and a block with the singleton record.

Once such a \qdrt is constructed, we loop through all produced leaves, and
partition them into two sets: those with size $\geq b$ and those with size $< b$
(the original constraint).  We then replicate each block in the small-size set to
any of its \emph{neighboring} blocks in the large-size set.  (We define
two blocks to be neighboring to mean that their hypercubes having one boundary
in common at some dimension $d$.)  This ensures that, with minor modifications
to node metadata, the semantic descriptions preserve completeness.
With this scheme, our algorithms could reach the optimal partitioning for the
scenario in Figure~\ref{fig:propeller} at virtually no extra storage cost.

\revision{
\subsubsection{Data and Query Routing}

Data routing occurs as before, with a row routed to all matching blocks. Rows landing in replicated blocks are simply copied to every replica. For query processing, our candidate
set of blocks to be touched includes all blocks that overlap with the query rectangle. However, we can leverage the completeness property of blocks to prune out blocks that
are redundant. For example, a query that asks only for the centre rectangle (with the singleton record) in the example above does not have to fetch all blocks, \emph{even though the min-max index for all four blocks includes it}. This is because of our semantic descriptions and completeness properties: we can prune away the other blocks because the first block completely covers the query rectangle.

Once we allow overlap, the set of blocks scanned when evaluating a query may contain duplicate rows which could result in duplicates in the query result. To avoid this, when scanning block ID $i$, we simply ignore tuples that match the semantic description of any selected block with a lower block ID.
}

\begin{figure}[t!]
\centering
\includegraphics[width=.55\columnwidth]{figs/propeller.pdf}
% \vspace{-.05in}
\caption{\small A scenario where significant data skipping is gained by
  replicating a single record.  Each query selects $N+1$ records. The queries
  only overlap in the one tuple placed at the center. If the space is naively
  cut in a binary fashion, 3 out of 4 queries each reads $N$ extra tuples.  By handling overlap, \qdrt
  replicates the singleton record to all four N-record regions, so no queries
  touch unnecessary records.\label{fig:propeller}}
\end{figure}

\subsection{Data Replication: two-tree approach}

Full-copy data replication is a complimentary approach to overlap in utilizing extra storage. The extension for \qdrt construction to support such replication is natural.

First, we learn (using our greedy or RL algorithm) a \qdrt, $T_1$, optimized for the full workload $W$. Then, we can in fact build a \emph{second} \qdrt, $T_2$, tailored for the queries that experience the worst skippability under tree $T_1$. The second tree is a logical copy of the entire dataset. By routing queries in $W$ through tree $T_1$ (Section~\ref{sec:query-proc}), we can collect the worst $K$ queries, say $W' \subseteq W$.  We then start producing $T_2$ for $W'$. Additionally, the first tree $T_1$ can be \emph{re-built} and
re-optimized for the complement, $W-W'$, possibly iterating until convergence. As a variant, we may designate one tree as the primary data copy and prune the other tree to eliminate blocks that are not covered by any query for that tree, to save space. The idea may also be extended to more than two trees if needed. Exploring such extensions is a rich area for future work.

%In our preliminary experiments, we find that the two-tree approach can indeed
%provide additional data skipping gains, even for the highly uniform synthetic
%workload TPC-H. We plan to study two-tree replication on real-world data as
%part of our future work.

% \todo{write?}

% \qdrt allow
% With the abundance of cheap storage in the cloud, one desirable feature for an
% analytics system is to trade space for potentially faster execution time.  A
% fruitful line of work has dedicated to this problem, e.g., materialized views,
% which we review in related work.  We now discuss how \qdrt can also naturally
% support replicating data.


% \subsection{Discussion}

% \noindent
% {\bf Handling Many Queries.}
% %
% A large number of queries implies many candidate cuts, which can slow down the QDRT learning process. To address this problem, we can merge similar queries based on bounding box overlap. For instance, if the joint cardinality of two queries is close to the sum of their individual cardinalities, it is safe to consider them as a single query for the purpose of QDRT construction.

% \noindent
% {\bf Handling Parameterized Queries.}
% %
% In practice, users register query templates with the DBMS, and execute the query for different parameters. To handle such workloads, for each query template, we simply use a representative sample of query instances based on parameters observed in the recent history.

% \noindent
% {\bf Handling Large Datasets.}
% %
% We need to route tuples and compute the benefit of every candidate routing tree. This can be expensive for large datasets. We can leverange standard prior techniques such as sampling to reduce the runtime of the QDRT learning procedure, based on the time budget and compute resources available for the learning process.

% \noindent
% {\bf Optimizing RL Runtime.}
% %
% Describe systems tricks to speed up RL.

% LocalWords:  nationkey shipdate commitdate receiptdate

